Learning to Learn to be Right for the Right Reasons

Improving model generalization on held-out data is one of the core objectives in commonsense reasoning. Recent work has shown that models trained on the dataset with superficial cues tend to perform well on the easy test set with superficial cues but perform poorly on the hard test set without superficial cues. Previous approaches have resorted to manual methods of encouraging models not to overfit to superficial cues. While some of the methods have improved performance on hard instances, they also lead to degraded performance on easy instances. Here, we propose to explicitly learn a model that does well on both the easy test set with superficial cues and hard test set without superficial cues. Using a meta-learning objective, we learn such a model that improves performance on both the easy test set and the hard test set. By evaluating our models on Choice of Plausible Alternatives (COPA) and Commonsense Explanation, we show that our proposed method leads to improved performance on both the easy test set and the hard test set upon which we observe up to 16.5 percentage points improvement over the baseline.

==> tables/contextless_setting.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{1}{c}{Model} & \multicolumn{1}{c}{Cs-Ex}  \\ \midrule
Random  & 33.3 \\
RoBERTa-base & 82.7 $_{\pm0.1}$ \\
RoBERTa-large & 85.3 $_{\pm0.4}$ \\ \bottomrule
\end{tabular}
\caption{Average accuracy with standard deviation of models trained on the answers only.}
\label{tab:answer-only-baseline}
\end{table}

==> tables/easy_hard_split.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\centering
\begin{tabular}{@{}lrr@{}}
\toprule
Dataset & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Hard} \\ \midrule
COPA*   & 190                      & 310                      \\
Cs-Ex   & 1572                     & 449                      \\ \bottomrule
\end{tabular}
\caption{Easy and Hard statistics for COPA and Commonsense Explanation (Cs-Ex). COPA* we use the same split in \citet{kavumba-etal-2019-choosing}}
\label{tab:easy-hard-split}
\end{table}

==> tables/old_rel.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[t]
\centering
\adjustbox{max width=\textwidth}{%
\begin{tabular}{@{}lllccc@{}}
\toprule
Model                          & Data                   & Training   & \multicolumn{1}{l}{Easy} & \multicolumn{1}{l}{Hard} & \multicolumn{1}{l}{Overall} \\ \midrule
\multirow{3}{*}{RoBERTa-large} & COPA                   & normal     & 90.5                     & 83.9                     & 86.4                        \\
                               & B-COPA                 & normal     & 90.0                     & 88.1                     & 88.8                        \\
                               & COPA                   & meta-train & \textbf{92.6}            & \textbf{89.7}            & \textbf{90.8}               \\ \cmidrule(l){1-6}
\multirow{3}{*}{RoBERTa-base}  & COPA                   & normal     & 80.0                     & 71.3                     & 74.6                        \\
                               & B-COPA                 & normal     & 78.4                     & 78.1                     & 78.2                        \\
                               & COPA                   & meta-train & \textbf{87.9}            & \textbf{78.4}            & \textbf{82.0}               \\\midrule
\multirow{2}{*}{RoBERTa-large} & \multirow{2}{*}{Cs-Ex} & normal     & 98.0                     & 79.1                     & 93.8                        \\
                               &                        & meta-train & \textbf{98.9}            & \textbf{87.1}            & \textbf{96.2}               \\ \cmidrule(l){1-6}
\multirow{2}{*}{RoBERTa-base}  & \multirow{2}{*}{Cs-Ex} & normal     & 95.0                     & 62.1                     & 87.7                        \\
                               &                        & meta-train & \textbf{97.6}            & \textbf{78.6}            & \textbf{93.4}               \\ \bottomrule
\end{tabular}
} %adjust box
\caption{Accuracy on Easy and Hard instances}
\label{tab:main-results}
\end{table*}
